Spatial-Temporal Mixture-of-Graph-Experts for Multi-Type Crime Prediction

As various types of crime continue to threaten public safety and economic development, predicting the occurrence of multiple types of crimes becomes increasingly vital for effective prevention measures. Although extensive efforts have been made, most of them overlook the heterogeneity of different crime categories and fail to address the issue of imbalanced spatial distribution. In this work, we propose a Spatial-Temporal Mixture-of-Graph-Experts (ST-MoGE) framework for collective multiple-type crime prediction. To enhance the model's ability to identify diverse spatial-temporal dependencies and mitigate potential conflicts caused by spatial-temporal heterogeneity of different crime categories, we introduce an attentive-gated Mixture-of-Graph-Experts (MGEs) module to capture the distinctive and shared crime patterns of each crime category. Then, we propose Cross-Expert Contrastive Learning(CECL) to update the MGEs and force each expert to focus on specific pattern modeling, thereby reducing blending and redundancy. Furthermore, to address the issue of imbalanced spatial distribution, we propose a Hierarchical Adaptive Loss Re-weighting (HALR) approach to eliminate biases and insufficient learning of data-scarce regions. To evaluate the effectiveness of our methods, we conduct comprehensive experiments on two real-world crime datasets and compare our results with twelve advanced baselines. The experimental results demonstrate the superiority of our methods.

==> algorithm.tex <==

\begin{algorithm}
\caption{Optimization Process of MVSTGL}
\label{alg}
\begin{algorithmic}[1]
    \STATE \textbf{Input:} Training instances $D$ $\{ (x^{(i)}, y^{(i)}) \}$, learning rate $\alpha$, maximum iteration $iter_{max}$, warm up iterations $iter_{warm_up}$;
    \STATE Initialize the balance coefficients $\lambda_{c,k}=1$, for $c=1,2,...,C$ and $k=1,2,...,K$, initialize the historical loss buffer $\mathcal{B}$ as an empty set.
    \FOR{$t = 1$ to $iter_{max}$}
        \FOR{each mini-batch $(X, Y) \in D$}
            %\STATE $\hat{\bm{X}} \gets $ Equation \ref{12}
            \FOR{$c=1,2,...,C$ and $k=1,2,...,K$}
                \IF{$epoch > iter_{warm_up}$}
                
                    \STATE $\mathcal{L}(t-1)_{c,k}$, $\mathcal{L}(t-2)_{c,k} \gets \mathcal{B}[t-1]_{c,k}, \mathcal{B}[t-2]_{c,k}$
                     
                    \STATE $\lambda_c(t), \lambda_{c,k}(t) \gets $ Equation \ref{eq13}
                \ENDIF
                
            \ENDFOR

                \STATE //Calculate the reweighted loss 
                \STATE $\mathcal{L}(t)\gets$ Equation \ref{eq21}, for $c=1,2,...,C$ and $k=1,2,...,K$
                \STATE Compute gradients with loss $\mathcal{L}(t)$ and update parameters with the optimizer

                \STATE //Update the historical loss buffer $\mathcal{B}$
                \STATE $\mathcal{B}[t]_{c,k} \gets \mathcal{L}(t)_{c,k}$
        \ENDFOR
    \ENDFOR
    \STATE \textbf{Output:} Optimized MVSTGCL;
\end{algorithmic}
\end{algorithm}

==> tables/table_notations.tex <==
\begin{table}
  \caption{Description of Key Notations}
  \label{table_notation}
  \centering
  \begin{tabular}{ccl}
    \hline
    \textbf{Notations} & Description\\
    \hline
    $R,T,C$ & Number of regions, timeslots, crime categories.\\
    $r,t,c$ & Index of regions, timeslots, crime categories. \\
    $\bm{X}_{r,t,c}$ & Number of crimes at region $r$, timeslot $t$, and category $c$.  \\
    %$\bm{H}^{(G)}$ & Output representations of GCNs.  \\
    %$\bm{H}^{(T)}$ & Output representations of TCNs.  \\
    $\bm{H}^{(S)}_c$ & Representations from $c$-th category-specific expert.  \\
    $\bm{H}^{(U)}$ & Representations from the universal expert.  \\
    $\bm{H}^{(F)}_c$ & The fusion result of $\bm{H}^{(M)}$ and $\bm{H}^{(U)}_c$.  \\
    $\tilde{H}_c$ & The corrupt representation for contrastive learning.\\
    %$\bm{M}^{c,k}$ & Mask of region cluster $k$ with crime type $c$.\\
    \hline
  \end{tabular}
\end{table}

